Game-Theoretic Planning for Autonomous Driving among Risk-Aware Human Drivers

We present a novel approach for risk-aware planning with human agents in multi-agent traffic scenarios. Our approach takes into account the wide range of human driver behaviors on the road, from aggressive maneuvers like speeding and overtaking, to conservative traits like driving slowly and conforming to the right-most lane. In our approach, we learn a mapping from a data-driven human driver behavior model called the CMetric to a driver's entropic risk preference. We then use the derived risk preference within a game-theoretic risk-sensitive planner to model risk-aware interactions among human drivers and an autonomous vehicle in various traffic scenarios. We demonstrate our method in a merging scenario, where our results show that the final trajectories obtained from the risk-aware planner generate desirable emergent behaviors. Particularly, our planner recognizes aggressive human drivers and yields to them while maintaining a greater distance from them. In a user study, participants were able to distinguish between aggressive and conservative simulated drivers based on trajectories generated from our risk-sensitive planner. We also observe that aggressive human driving results in more frequent lane-changing in the planner. Finally, we compare the performance of our modified risk-aware planner with existing methods and show that modeling human driver behavior leads to safer navigation.

==> Sections/Theory.tex <==
\section{Game-Theoretic Planning is NP-Complete}
\label{sec: np-complete}

In the previous section, we described a method to compute game-theoretically optimal turn-based orderings which help in navigating traffic scenes in a collision- and deadlock-free way. $\sigma_{\textsc{opt}}$ is based on driver behavior. Driver behavior is what we are going to refer to as an attribute.

\begin{definition}
An attribute is a mapping $\bm{\Lambda}: \mathcal{A} \rightarrow \mathbb{R}$.
\end{definition}

\noindent $\bm{\Lambda}$ is an element of an infinitely countable set. We define such a set as $\bm{\Upsilon} = \{ \bm{\Lambda}_1, \bm{\Lambda}_2, \ldots, \}$, where $\bm{\Lambda}$ is indexed by the natural numbers. Then the mapping corresponding to driver behavior may be indexed by some constant $d \in \mathbb{N}$ to produce a mapping $\bm{\Lambda}_d$.

Now the natural question may be asked - what if we were to choose a different attribute than driver behavior, (any $j \neq d \in \mathbb{N}$)? Can a different sorting strategy be used to sort drivers and therefore come up with a different turn-based ordering that is also game-theoretically optimal?

We will show that finding the attribute that results in a game-theoretically optimal turn-based ordering is NP-complete.

\subsection{Model $\mathcal{M}$}
\begin{itemize}
    \item Given $N$ human drivers, we want to identify first-goers, second-goers, $\ldots$, $k^\textrm{th}$-goers etc. This amounts to making $k$ clusters, $\mathcal{C}_1,\mathcal{C}_2,\ldots,\mathcal{C}_k$, where $\mathcal{C}_i$ consists of the drivers who will move on the $i^\textrm{th}$ turn while maintaining game-theoretic optimality.
    
    \item Given a set of attribute mappings $\bm{\Upsilon} = \{ \bm{\Lambda}_1, \bm{\Lambda}_2, \ldots\}$ where $\bm{\Lambda}_j: \mathcal{A} \rightarrow \mathbb{R}$. No other information is known about an agent. $\bm{\Lambda}_j(a_i)$ can be computed in polynomial time.
    
    
    \item We want to find the attribute mapping, say $\bm{\Lambda}_j \in \bm{\Upsilon}$, such that $\bm{\Lambda}_j(a_1) > \bm{\Lambda}_j(a_1)>\ldots>\bm{\Lambda}_j(a_k) \ \forall a_1,a_2,\ldots,a_k \in \mathcal{C}_1,\mathcal{C}_2,\ldots,\mathcal{C}_k$. 
    
    \item Assume fixed number of clusters ($k \geq 2$) but number of agents ($N$) is part of input.
    
    \item $P(\bm{\Lambda}_j (a_i) | a_i)$ is unknown.
    
\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width = \linewidth]{img/Appendix/NP-complete digram.png}
    \caption{Attributes in \model.}
    \label{fig: np-complete}
\end{figure}


\subsection{Result}

\begin{theorem}
Finding a game-theoretically optimal attribute is NP-complete.
\end{theorem}

\begin{proof}
We reduce \texttt{SAT} to our model.  Each cluster is a circuit composed of the corresponding clause.


\begin{enumerate}

    \item $\mathcal{M} \in \textrm{NP}$. Proof - Given $N$ agents, $k$ clusters, and an attribute mapping $\bm{\Lambda}_j, j\in \mathbb{N}$, checking the mapping takes $\bigO{\floor*{\frac{N}{k}}^{k}}$. Note that $\mathcal{M}$ is $\texttt{EXPTIME}$ if $k$ is not fixed.

    \item $\phi \implies \mathcal{M}$: Let $\phi$ be satisfied by $\hat j = x_1x_2\ldots x_n$ and let $j$ be the decimal form of $\hat j$. The attribute map is $\bm{\Lambda}_j(a_i) = (j + k - i)*\texttt{bool}(\mathcal{C}_i) \in \mathbb{R} \ \forall a_i \in \mathcal{C}_i, i \in [1,k]$. Therefore, $\bm{\Lambda}_j(a_i)$ can be either $j+k-i$ or $0$. Each agent in $\mathcal{C}_i$ is represented by $a_i \gets (l, (j+k-i)*\texttt{bool}(\mathcal{C}_i))$ where $l$ represents the literal in the $i^\textrm{th}$ clause. 
    
    Now, $j$ satisfying $\phi$ implies that there exists a game-theoretically optimal attribute mapping $\bm{\Lambda}$ that fits model $\mathcal{M}$. Indeed, such a mapping is $\bm{\Lambda}_j(a_i) = (j + k - i)*\texttt{bool}(\mathcal{C}_i) \in \mathbb{R} \ \forall a_i \in \mathcal{C}_i, i \in [1,k]$. To see why, pick any agent from $\mathcal{C}_1$. Since every clause is true, $\bm{\Lambda}_j(a_1) = j+k-1$. Similarly, any agent from $\mathcal{C}_2$ will have an attribute value of $j+k-2 < j+k-1$. So on up til $\mathcal{C}_k$ in which each agent has attribute value $j$.
    
    \item $\mathcal{M} \implies \phi$: Assume there exists a game-theoretically optimal attribute $\bm{\Lambda}_j$. $\hat j = j$ if $j\in [1,2^n]$ else $\hat j = j\bmod 2^n$. Then $\bm{\Lambda}_j(a_1) > \bm{\Lambda}_j(a_2)>\ldots>\bm{\Lambda}_j(a_k) \ \forall a_1,a_2,\ldots,a_k \in \mathcal{C}_1,\mathcal{C}_2,\ldots,\mathcal{C}_k$ and $j\in \mathbb{N}$. This automatically implies each cluster has a truth value of $1$. To see why, assume that $\phi$ is not satisfied. Then there exist one or more clusters whose truth value is $0$. Assume that such a cluster is $\mathcal{C}_i$. Then each agent in $\mathcal{C}_i$ has an attribute value of $0$ contradicting the game-theoretic optimality ($0 > j+k-(i+1)$ is a contradiction since $j\in \mathbb{N}$ and $k \geq 2$). Therefore, each clause/cluster has a truth value of $1$ implying $\phi$ is satisfied.
    
    % To obtain $\hat j$, note that if $\hat j = j$ if $j\in [1,2^n]$. Otherwise, $\hat j = j\mod 2^n$
\end{enumerate}

% \noindent Think of the solution code as ``lighting up'' the clusters (setting them to 1). The problem is we do not know which attribute results in the desired order (lights up all the clusters). 
\end{proof}

\noindent This means that given a traffic scenario such as an intersection or roundabout with $k$ arms that requires the interaction of $N$ agents (nothing known about them), unless $P = NP$, collision- and deadlock-free navigation cannot be guaranteed without relaxing some of the constraints or making assumptions heuristically.

\subsection{Heuristic algorithms to solve $\mathcal{M}$}

Recall that the end goal is to compute $\sigma_{\textsc{opt}}$ which, as per the discussion in this section, depends on the optimal attribute mapping $\bm{\Lambda}_j$. We have proven that finding the value of $j$ is NP-complete. However, one can design heuristic algorithms to solve $\mathcal{M}$. The basic premise of such an algorithm is to relax some of the constraints above associated with $\mathcal{M}$.

For example, \model~is one such heuristic algorithm where we relax the last constraint, \textit{i.e.}, we use an attribute mapping with a known probability distribution, $P(\bm{\Lambda}_j (a_i) | a_i)$. Consider an aggressive agent $a_{\textsc{aggressive}}$. Then it is known with high probability that $\bm{\Lambda}_j (a_{\textsc{aggressive}}) = t$ for some fixed $t$. Monetary-based auction methods are another instance of a heuristic multi-agent game-theoretic planning algorithms for computing game-theoretical turn-based orderings. In these type of methods, it is assumed that agents are given a known monetary budget. Consequently, the mapping is provided by an oracle and is not known to be computed in polynomial time. Such auctions work by relaxing the second constraint.


==> Tables/accuracy.tex <==


% \begin{table*}[t]
% \caption{\textbf{Comparison with SOTA:} We compare the percentage of collisions and deadlocks with two planning baselines designed for uncontrolled intersections.}
% \centering
% % \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccccccc} 
% \toprule
% &&&\multicolumn{7}{c}{$4$-way intersection}&&&\\

% Method \Tstrut & \multicolumn{2}{}{$2$ vehicles} \Bstrut &   \multicolumn{2}{}{$3$ vehicles} & \multicolumn{2}{}{$4$ vehicles} \\
% \midrule
% Roh et al.~\cite{roh2020multimodal} & $30$  & - &&&& \\
% Tian et al.~\cite{tian2020game} & $20$   & $20$ &&&&\\
% Li et al.~\cite{li2020game} && &&&&\\
% \textbf{\model} &      $\textbf{0}$       & $\textbf{0}$ &&&&\\
% \bottomrule
% \end{tabular}
% % }
% \label{tab: accuracy}
% \vspace{-10pt}
% \end{table*}

% \begin{table*}
% \centering
% \caption{\textbf{Error rate analysis with grouping:}   }
% \resizebox{\linewidth}{!}{%
% \makebox[\textwidth][c]{
% \begin{tabular}{cc|ccc|ccc|ccc|ccc|ccc|ccc}
% \toprule[1.1pt]
%  Methods   & &
% \multicolumn{3}{c|}{Smooth Navigable Region}
% &
% \multicolumn{3}{c|}{Rough Navigable Region}
% &
% \multicolumn{3}{c|}{Bumpy Region}      
% &
% \multicolumn{3}{c|}{Forbidden Region}
% &
% \multicolumn{3}{c|}{Obstacle}
% &
% \multicolumn{3}{c}{Background}   
% \\
% \midrule
% x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x & x \\

% %                     &
% % \multicolumn{2}{c}{CS-LSTM }         &
% % \multicolumn{2}{c}{TraPHic  }         &
% % \multicolumn{2}{c}{Social-GAN  }         &
% % \multicolumn{2}{c}{GRIP  }         &
% % \multicolumn{2}{c}{S1 Only }  &
% % \multicolumn{2}{c}{S1 + S2 \Tstrut }            \\


% % \midrule
% % &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE &
% % ADE & FDE \\
% % \midrule
% % \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|}z
% % Lyft (5 sec.)           &   4.423  &  8.640  & 5.031  &  9.882   &  7.860  &  14.340  & -  &  - & 5.77  &  11.20  &  \textbf{2.65} &  \textbf{2.99}\\ 
% % Argoverse (5 sec.)      &    1.050  &  3.085  & 1.039  &  3.079   &  3.610   &  5.390  & -  &- &  2.40 &  3.09  &  \textbf{0.99} &  \textbf{1.87} \\ 
% % Apolloscape (3 sec.)    &    2.144  &  11.699  & 1.283  &  11.674  & 3.980  & 6.750  & 1.25 &  2.34  & 2.14  & 9.19  &  \textbf{1.12} &  \textbf{2.05}\\ 
% % NGSIM (5 sec.)  &   7.250&10.050  & 5.630&9.910  & 5.650&10.290  & 1.61  &  3.16  &  1.31  &  2.98  &\textbf{0.40}  & \textbf{1.08}\\ 


% \bottomrule[1.1pt]
% \end{tabular}
% }
% }
% \label{tab: accuracy}
% % \vspace{-15pt}
% \end{table*}


\begin{table*}[t]
% \newcolumntype{Z}{S[table-format=2.2,table-auto-round]}
\caption{\textbf{Comparison with SOTA:} We compare the percentage of collisions, deadlocks, and overall success rate with state-of-the-art planning methods designed for uncontrolled and unsignaled intersections. We reduce the collision frequency by up to $30\%$ (versus Roh et al.~\cite{roh2020multimodal} for $4$ vehicles at a $4$-way intersection). The \xmark~symbol indicates that results for that setting were not provided by the method.
}
\centering
% \setlength{\tabcolsep}{3mm}
% \ra{1.05}
% \Large
% \begin{adjustbox}{max width=\textwidth}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccccccccccccc@{}}
  \toprule[1.5pt]
   \multirow{4}[3]{*}{Methods}&&&&&&$4-$way Intersection&&&&&&\\ 
  \cmidrule[1pt](l{3mm}r{3mm}){3-13}   &&
  \multicolumn{3}{c}{$2$ Vehicles}&& 
  \multicolumn{3}{c}{$3$ Vehicles}&&  
  \multicolumn{3}{c}{$4$ Vehicles}\\
  \cmidrule(l{3mm}r{3mm}){3-5} 
  \cmidrule(l{3mm}r{3mm}){7-9} 
  \cmidrule(l{3mm}r{3mm}){11-13}
   && {Collisions (\%)} & {Deadlocks (\%)} & Success (\%) &&  {Collisions (\%)} & {Deadlocks (\%)} & Success (\%) &&  {Collisions (\%)} & {Deadlocks (\%)} & Success (\%)\\
%   \midrule
%   \midrule
\midrule
%  &&&&&&$4-$way Intersection Groups&&&&&&\\ 
%   \midrule
  Liu et al.~\cite{liu2020decision} && 
    \xmark & \xmark & \xmark && 
    \xmark & \xmark & \xmark && 
    $6.25$ & \xmark & $93.75$  \\ 
  Isele et al.~\cite{isele2018navigating} && 
    \xmark & \xmark & \xmark && 
    \xmark & \xmark & \xmark && 
    $7.1$ & $0.2$ & $92.80$  \\ 
Kai et al.~\cite{Kai2020AMR} && 
    $0$ & $0$ & $100$ && 
    \xmark & \xmark & \xmark && 
    $3.70$ & $0$ & $96.30$  \\ 
    
  Li et al.~\cite{li2020game} && 
    $0$ & $0$ & $100$ && 
    \xmark & \xmark & \xmark && 
    $0$ & $0$ & $100$  \\ 
  Roh et al.~\cite{roh2020multimodal} &&
    $2$ & \xmark & $98$& &$2$ & \xmark & $98$ && $30$ & \xmark & $70$   \\ 
  Tian et al.~\cite{tian2020game} && 
    $0-10$ & $0$ & $>90$ && 
    $0-10$ & $0$ & $>90$ && 
    $0-10$ & $0$ & $>90$  \\ 
  \model  && 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ && 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ && 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$  \\ 
  \midrule
  
 \midrule
%   \midrule
    \multirow{4}[3]{*}{Methods}&&&&&&$> 4-$way Intersection&&&&&&\\ 
   \cmidrule[1pt](l{3mm}r{3mm}){3-13} 
 &&
  \multicolumn{3}{c}{$6$ Vehicles}&& 
  \multicolumn{3}{c}{$8$ Vehicles}&&  
  \multicolumn{3}{c}{$10$ Vehicles}\\
  \cmidrule(l{3mm}r{3mm}){3-5} 
  \cmidrule(l{3mm}r{3mm}){7-9} 
  \cmidrule(l{3mm}r{3mm}){11-13}
   && {Collisions (\%)} & {Deadlocks (\%)} & Success (\%) &&  {Collisions (\%)} & {Deadlocks (\%)} & Success (\%) &&  {Collisions (\%)} & {Deadlocks (\%)} & Success (\%)\\
  \midrule
  Li et al.~\cite{li2020game} && 
    $0-10$ & $0-10$ & $>90$ && 
    $0-20$ & $0-20$ & $>80$ && 
    $0-20$ & $0-20$ & $>80$  \\ 
  \model  && 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ && 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$ && 
    $\textbf{0}$ & $\textbf{0}$ & $\textbf{100}$  \\ 


  \bottomrule[1.5pt]
\end{tabular}
}
% \end{adjustbox}
% \vspace{-6mm}
\label{tab: accuracy}
%   \vspace{-10pt}
\end{table*}

==> Tables/benefits.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Benefits of \model~over prior work in planning.}}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}

\toprule
%  &  &  & \multicolumn{2}{c}{Our CMetric Measures}\\

% \cline{4-5}
Problem Setting & Approach & Methods & Assumptions/Limitations & Benefits\\
\midrule
\multirow{2}{*}{Single-agent planning with dynamic obstacles} & Geometric Methods  && \\
                                             & Learning-based Methods && \\


\multirow{2}{*}{Multi-agent planning} & Game theory  && \\
                                             & Auctions && \\
 
\bottomrule
\end{tabular}
}
\label{tab: benefits}

\end{table*}

==> Tables/centrality.tex <==
\begin{table}%[tbhp]
\centering
\caption{Relationship between centrality and driving behavior.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lc}
\toprule
Centrality & Specific Style/Indicator  \\
\midrule
Degree & Overspeeding \\
Closeness  & Weaving, Overtaking, Sudden Lane Changes \\
Eigenvector & Overspeeding, Weaving\\
% Laplacian Centrality &  Degree of ``agitation'' &  High (Agg.) or Low (Con.)\\
\bottomrule
\end{tabular}
}
\label{tab: centrality_relationship}
\vspace{-10pt}
% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
\end{table}

==> Tables/notation.tex <==
\begin{table}[t]
  \caption{Symbols and notations used in this paper.}
  \label{tab: notation}
  \centering
  \resizebox{.7\columnwidth}{!}{%
  \begin{wraptable}{r}{5.5cm}
  \begin{tabular}{cl}
  \toprule
    Symbol  & Description \\
    \midrule
    $n$ & Number of traffic-agents.\\
    $a_i$ & $i^\textrm{th}$ active agent.\\
    $\mathcal{A}$ & Set of active agents. \\
    $\zeta$ & CMetric-based behavior profile (Section~\ref{subsec: cmetric_background}). \\
    $\sigma$ & Turn-based ordering (Definition~\ref{def: turn_based_ordering}). \\
    $\sigma_{\textsc{opt}}$ & Optimal turn-based ordering (Definition~\ref{def: optimal_turn_based_ordering}). \\
    $b_i$ & Bid of the $i^\textrm{th}$ active agent.\\
    $b_{-i}$ & Bid of every agent except the $i^\textrm{th}$.\\
    $v_i$ & Private valuation of the $i^\textrm{th}$ active agent.\\
    $u_i(\cdot)$ & Utility of the $i^\textrm{th}$ active agent.\\
    $t_i$ & Time taken by the $i^\textrm{th}$ active agent \\
    & to navigate the traffic scenario.\\

    \bottomrule
  \end{tabular}
  \end{wraptable} 
  }
%   }
  \vspace{-15pt}
\end{table}


==> Tables/parameters.tex <==
\begin{table}[h]
\caption{IDM and MOBIL parameters used for Conservative and Aggressive vehicle classes}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{clcc} 
\toprule
Model & Parameter \Tstrut & Conservative \Bstrut &   Aggressive \\
\hline
\multirow{4}{*}{IDM}& Time gap ( $T$) \Tstrut & 1.5s      & 1.2s \\
 &Min distance ($s_0$) & 5.0 $m$ & 2.5 $m$ \\
&Max comfort acc. ($a$)     & 3.0 $m/s^2$ & 6.0 $m/s^2$\\
&Max comfort dec. ($b$) & 6.0 $m/s^2$               &  9.0 $m/s^2$ \\
\midrule
\multirow{3}{*}{MOBIL}& Politeness ($p$) & 0.5     & 0\\
& Min acc gain ($\Delta a_{th}$) & 0.2 $m/s^2$ & 0 $m/s^2$ \\
& Safe acc limit ($b_{safe}$) & 3.0 $m/s^2$ & 9.0 $m/s^2$\\
\bottomrule
\end{tabular}
}
\label{tab: parameters}
\vspace{-10pt}
\end{table}


==> img/Real_World.tex <==
\begin{figure*}[t]
\centering
% \resizebox{.9\linewidth}{!}{
    % \begin{subfigure}[h]{.6\linewidth}
    \begin{subfigure}[h]{\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/real_world/white_black.png}
    \caption{$\sigma_W = 1, \sigma_B = 2$, TTG $= 7$ seconds.}
    \label{fig: white_black}
    % \vspace{5pt}
  \end{subfigure}
  %
  \begin{subfigure}[h]{\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/real_world/white_silver.png}
    \caption{$\sigma_W = \sigma_S = \textrm{\xmark}$, TTG $= 15$ seconds.}
    \label{fig: white_silver}
    % \vspace{5pt}
  \end{subfigure}
  %
%     \begin{subfigure}[h]{0.32\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/real_world/wb3.png}
%     \caption{B follows next.}
%     \label{fig: argo3}
%     \vspace{5pt}
%   \end{subfigure}
% %
%     \begin{subfigure}[h]{0.32\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/real_world/ws1.png}
%     \caption{S and W both stop.}
%     \label{fig: argo1}
%   \end{subfigure}
%   %
%   \begin{subfigure}[h]{0.32\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/real_world/ws2.png}
%     \caption{W moves first.}
%     \label{fig: argo2}
%   \end{subfigure}
%   %
%     \begin{subfigure}[h]{0.32\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/real_world/ws3.png}
%     \caption{S follows next.}
%     \label{fig: argo3}
%   \end{subfigure}
%   \end{subfigure}
  %
%   \begin{subfigure}[h]{0.35\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/real_world/real_world.png}
%     \caption{}
%     \label{fig: argo3}
%   \end{subfigure}
%
  %
%   }
\caption{\textbf{Demonstrating \model~with Human Drivers:} In Figure~\ref{fig: white_black}, the driver of the white (W) vehicle is aggressive while the driver of the black (B) vehicle is conservative. \model~computes a turn-based ordering that determines the black agent should yield to the white vehicle, which would pass first. In Figure~\ref{fig: white_silver}, we do not perform game-theoretic planning and consequently, both drivers are unsure of who should move first. In this case, both the white (W) and silver (S) agents stop and after a delay of $8$ seconds, the white vehicle moves first (due to the inherently aggressive nature of the driver) followed by the silver vehicle.}
  \label{fig: real_world}
%   \vspace{-15pt}
\end{figure*}

==> img/cover/cover.tex <==
\begin{figure}[t]
\centering
% \resizebox{.9\linewidth}{!}{
    \begin{subfigure}[t]{.45\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/cover/cover_aggressive.png}
    \caption{\textbf{Without \model:} Aggressive agents at an unsignaled intersection move together resulting in collision.}
    \label{fig: cover1}
    % \vspace{10pt}
  \end{subfigure}
  %
  \begin{subfigure}[t]{.45\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/cover/cover_aggressive_gameplan.png}
    \caption{\textbf{\model:} Red agent moves first followed by yellow agent. The numbers correspond to the turn-based ordering.}
    \label{fig: cover2}
    % \vspace{10pt}
  \end{subfigure}
  %
\begin{subfigure}[t]{.45\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/cover/cover_conservative.png}
    \caption{\textbf{Without \model:} Conservative agents at an unsignaled intersection are uncertain and enter a deadlock.}
    \label{fig: cover3}
    % \vspace{10pt}
  \end{subfigure}
  %
  \begin{subfigure}[t]{.45\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/cover/cover_conservative_gameplan.png}
    \caption{\textbf{\model:} Order of movement is indicated by increasing numbers computed using our turn-based ordering.}
    \label{fig: cover4}
    % \vspace{10pt}
  \end{subfigure}
\caption{\textbf{\model:} We present the first approach of using driving behavior to compute a collision- and deadlock-free turn-based ordering (circled numbers) for non-communicating agents. Figure~\ref{fig: cover1} shows aggressive agents are more likely to collide due to their nature of moving first. Figure~\ref{fig: cover3} shows that conservative agents, on the other hand, are prone to entering a deadlock due to the uncertainty of the turn-based ordering. In our approach, we compute a turn-based ordering in which more aggressive agents are allowed to pass first. Thus, in Figure~\ref{fig: cover2}, the more aggressive red agent crosses the intersection followed by the more conservative yellow agent, thereby preventing a collision. In Figure~\ref{fig: cover4}, the order of aggressiveness is determined by the indicated numbers, and our approach can prevent deadlocks.}
  \label{fig: cover}
  \vspace{-15pt}
\end{figure}

==> img/merge_intersection.tex <==
\begin{figure}[t]
\centering
% \resizebox{.9\linewidth}{!}{
%     \begin{subfigure}[h]{0.282\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/Merge/merge_distance_single.png}
%     \caption{Merging: Minimum distance.}
%     \label{fig: merge_dist}
%     \vspace{10pt}
%   \end{subfigure}
  
%   \begin{subfigure}[h]{0.282\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/Merge/merge_behavior_single.png}
%     \caption{Merging: $2^\textrm{nd}$ agent yield \%.}
%     \label{fig: merge_yield}
%     \vspace{10pt}
%   \end{subfigure}
  %
    \begin{subfigure}[h]{0.45\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/Merge/Merge_Distance_Merge.png}
    \caption{Merging: minimum distance}
    \label{fig: merge_ttg}
    % \vspace{10pt}
  \end{subfigure}
% %
%     \begin{subfigure}[h]{0.282\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/Intersection/cross_distance_single.png}
%     \caption{Intersection: Minimum distance.}
%     \label{fig: cross_dist}
%   \end{subfigure}
%   %
%   \begin{subfigure}[h]{0.282\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/Intersection/cross_behavior_single.png}
%     \caption{Intersection: $2^\textrm{nd}$ agent yield \%.}
%     \label{fig: cross_yield}
%   \end{subfigure}
  %
    \begin{subfigure}[h]{0.45\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/Merge/Yield_Frequency_Merge.png}
    \caption{Merging: yielding frequency}
    \label{fig: cross_ttg}
  \end{subfigure}
%
%     \begin{subfigure}[h]{0.3\linewidth}
%     \includegraphics[width=\textwidth]{NeuRIPS2020/img/Roundabout/rb_time_comap_nogame.png}
%     \caption{Roundabout: Time to Goal.}
%     \label{fig: cross_ttg}
%   \end{subfigure}
  %
%   }
\caption{}
  \label{fig: merge_intersection}
%   \vspace{-15pt}
\end{figure}

% \begin{figure*}[t]
% 	\begin{center}
% 	    \subfloat[caption]{\includegraphics[width=0.283\textwidth]{NeuRIPS2020/img/Merge/merge_distance_single.png}\hspace{1pt}%
% 	    }
% 	    \subfloat[caption]{\includegraphics[width=0.283\textwidth]{NeuRIPS2020/img/Merge/merge_behavior_single.png}\hspace{1pt}%
% 	    }
% 	    \subfloat[caption]{\includegraphics[width=0.283\textwidth]{NeuRIPS2020/img/Merge/merge_time.png}
% 	    }
% 	\end{center}
% 	\begin{center}
% 	    \subfloat[caption]{\includegraphics[width=0.283\textwidth]{NeuRIPS2020/img/Intersection/cross_distance_single.png}\hspace{1pt}%
%   	    }
%   	    \subfloat[caption]{\includegraphics[width=0.283\textwidth]{NeuRIPS2020/img/Intersection/cross_behavior_single.png}\hspace{1pt}%
%   	    }
%   	    \subfloat[caption]{\includegraphics[width=0.283\textwidth]{NeuRIPS2020/img/Intersection/cross_time_comap_nogame.png}
%   	    }
% 	\end{center} 	 
% 	\caption{MAIN CAPTION}
% \end{figure*}

==> img/roundabout.tex <==
\begin{figure}[t]
\centering
% \resizebox{.9\linewidth}{!}{
    \begin{subfigure}[h]{.5\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/Roundabout/roundabout_behavior.png}
    \caption{Roundabout: $2^\textrm{nd}$ agent yield \%.}
    \label{fig: argo1}
  \end{subfigure}
  %
  \begin{subfigure}[h]{.4\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/Roundabout/rb_time_comap_nogame.png}
    \caption{Roundabout: Time to goal.}
    \label{fig: argo2}
  \end{subfigure}
%   }
\caption{\textbf{Min. Distance \& Second Agent \% Yield (Roundabouts):} We show results in the roundabout scenario. On each axis, the behavior of an agent ranges from conservative ($-5.0$) to aggressive ($+5.0$).}
  \label{fig: roundabout}
  \vspace{-10pt}
\end{figure}

==> img/sim_results/sim_merge.tex <==
\begin{figure}[t]
\centering
% \resizebox{.9\linewidth}{!}{
    \begin{subfigure}[h]{0.3\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/deadlock_merge.png}
    \caption{Deadlock (No\model).}
    \label{fig: merge_deadlock}
    % \vspace{10pt}
  \end{subfigure}
%
  \begin{subfigure}[h]{00.3\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/collision_merge.png}
    \caption{Collision (No\model).}
    \label{fig: merge_collision}
    % \vspace{10pt}
  \end{subfigure}
%
    \begin{subfigure}[h]{0.3\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/merge_no_deadlock_collision.png}
    \caption{\model~avoids collisions and deadlocks.}
    \label{fig: merge_no_coll_deadlock}
    % \vspace{10pt}
  \end{subfigure}
%   \caption{\textbf{Merging:} We visualize an instance of the results in Figure~\ref{fig: merge_intersection}. In Figures~\ref{fig: merge_collision} and~\ref{fig: merge_deadlock}, both agents are conservative and aggressive, respectively. This leads to a deadlock in the former case and collision in the latter case. In Figure~\ref{fig: merge_no_coll_deadlock}, the green agent is more aggressive than the red agent and \model tasks the red agent to yield to the green agent.}
\vspace{5pt}
    \begin{subfigure}[h]{0.3\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/conservative wait.png}
    \caption{Deadlock.}
    \label{fig: cross_deadlock}
  \end{subfigure}
  %
  \begin{subfigure}[h]{0.3\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/collisison.png}
    \caption{Collision.}
    \label{fig: cross_collision}
  \end{subfigure}
  %
    \begin{subfigure}[h]{0.3\linewidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/non-deadlock.png}
    \caption{\model.}
    \label{fig: cross_no_coll_deadlock}
  \end{subfigure}
%   }
\caption{\textbf{Visualizations:} We visually compare our algorithm with No\model. In Figures~\ref{fig: merge_deadlock} and~\ref{fig: cross_deadlock}, both agents are conservative while in Figures~\ref{fig: merge_collision} and~\ref{fig: cross_collision} both agents are aggressive. This leads to a deadlock in the first two scenarios while agents result in a collision in the latter two scenarios. In Figures~\ref{fig: merge_no_coll_deadlock} and~\ref{fig: cross_no_coll_deadlock}, the green agent is more aggressive than the red agent and \model~tasks the red agent to yield to the green agent. This demonstrates that our method can handle different type of agents.}
  \label{fig: simulation}
  \vspace{-10pt}
\end{figure}



==> img/sim_results/sim_results.tex <==
\begin{figure}[t]
\centering
    \begin{subfigure}[h]{0.32\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/conservative wait.png}
    \caption{Deadlock.}
    \label{fig: cross_deadlock}
  \end{subfigure}
  %
  \begin{subfigure}[h]{0.32\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/collisison.png}
    \caption{Collision.}
    \label{fig: cross_collision}
  \end{subfigure}
  %
    \begin{subfigure}[h]{0.32\columnwidth}
    \includegraphics[width=\textwidth]{NeuRIPS2020/img/sim_results/non-deadlock.png}
    \caption{\model.}
    \label{fig: cross_no_coll_deadlock}
  \end{subfigure}
%
  %
%   }
\caption{\textbf{Intersection:} We show simulation results in the intersection scenarios.}
  \label{fig: cross_sim}
%   \vspace{-10pt}
\end{figure}



==> table.tex <==
\begin{table}[H]
\centering
\caption{\textbf{Main Results:} We report the Average Displacement Error (ADE) and Final Displacement Error (FDE) for prior road-agent trajectory prediction methods in meters(m). Lower scores are better and \textbf{bold} indicates the SOTA. \textbf{Revisions:} Green colored cells indicate revised results for \textit{our} method while blue colored cells indicates revised results for the original implementations \textit{GRIP} and Social-GAN method.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule[1.1pt]
\multirow{2}{*}{Dataset \newline (Pred. Len.)}                       &
\multicolumn{2}{c}{CS-LSTM }         &
\multicolumn{2}{c}{TraPHic  }         &
\multicolumn{2}{c}{Social-GAN  }         &
\multicolumn{2}{c}{GRIP  }         &
\multicolumn{2}{c}{Ours (Stream 1 only)  }  &
\multicolumn{2}{c}{Ours (Both Streams)  }            \\
&
ADE & FDE &
ADE & FDE &
ADE & FDE &
ADE & FDE &
ADE & FDE &
ADE & FDE \\
\midrule
% \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|}z
Lyft (5 sec.)           &   4.423  &  8.640  & 5.031  &  9.882   &  \cellcolor{blue!20}7.860  &  \cellcolor{blue!20}14.340  & \cellcolor{blue!20}-  &  \cellcolor{blue!20}- & \cellcolor{green!20}2.23  &  \cellcolor{green!20}2.35  &  \cellcolor{green!20}\textbf{2.22} &  \cellcolor{green!20}\cellcolor{green!20}\textbf{2.33}\\ 
Argoverse (5 sec.)      &    1.050  &  3.085  & 1.039  &  3.079   &  \cellcolor{blue!20}3.610   &  \cellcolor{blue!20}5.390  & \cellcolor{blue!20}-  &\cellcolor{blue!20}- &  \cellcolor{green!20}2.06 &  \cellcolor{green!20}2.08  &  \cellcolor{green!20}\textbf{0.97} &  \cellcolor{green!20}\textbf{2.07} \\ 
Apolloscape (3 sec.)    &    2.144  &  11.699  & 1.283  &  11.674  & \cellcolor{blue!20} 3.980  & \cellcolor{blue!20} 6.750  & \cellcolor{blue!20}\textbf{1.25} &  \cellcolor{blue!20}2.34  & \cellcolor{green!20} 1.52  & \cellcolor{green!20} 1.56  &  \cellcolor{green!20}1.51 &  \cellcolor{green!20}\textbf{1.55}\\ 
NGSIM (5 sec.)  &   7.250&10.050  & 5.630&9.910  & \cellcolor{blue!20} 5.650&\cellcolor{blue!20}10.290  & \cellcolor{blue!20}1.61  &  \cellcolor{blue!20}3.16  &  \cellcolor{green!20}1.15  &  \cellcolor{green!20}1.17  &\cellcolor{green!20}\textbf{0.99}  & \cellcolor{green!20} \textbf{1.02}\\ 
\bottomrule[1.1pt]
\end{tabular}
}
\label{tab: accuracy}
% \vspace{-15pt}
\end{table}



